Zero-Shot Multi-Modal Artist-Controlled Retrieval and Exploration of 3D Object Sets

When creating 3D content, highly specialized skills are generally needed to design and generate models of objects and other assets by hand. We address this problem through high-quality 3D asset retrieval from multi-modal inputs, including 2D sketches, images and text. We use CLIP as it provides a bridge to higher-level latent features. We use these features to perform a multi-modality fusion to address the lack of artistic control that affects common data-driven approaches. Our approach allows for multi-modal conditional feature-driven retrieval through a 3D asset database, by utilizing a combination of input latent embeddings. We explore the effects of different combinations of feature embeddings across different input types and weighting methods.

==> sections/abstract.tex <==
%1or 2 sentences for background
When creating 3D content, highly specialized skills are generally needed to design and generate models of objects and other assets by hand.
%1/2 for problem
We address the problem of high-quality 3D asset retrieval from multi-modal inputs, including 2D sketches, images and text.
We use CLIP as it provides a bridge to higher-level latent features. We use these features to perform multi-modality fusion to address the lack of artistic control that affects common data-driven approaches.
%1/2 for what you did
Our approach allows for multi-modal conditional feature-driven retrieval through a 3D asset database, by utilizing a combination of input latent embeddings.
%1/2 for conclusion
We explore the effects of different combinations of feature embeddings across different input types and weighting methods.

==> sections/todo.tex <==
%!TEX root = main.tex
\section{To Do List}

One key point that separates our paper from other sketch-based retrieval methods (including zero-shot) is that other methods just return the one-to-one mapping between sketch and result.  Our work in contrast allows the user to tweak the mapping through the a combination of many inputs and or weighting of those inputs.  In this work we explore the effects of different combinations of inputs across different media types and weighting methods.

*Get everyone running and compiling code*

PAPER WRITING ADVICE/LINK:
https://dritchie.github.io/2017/10/12/three-phase-paper-writing.html


\begin{lstlisting}
What is novel in our research:
(1) possible contributions
(a) Multi-modal/input search
(b) Artistic control of retrieval
(c) semantic axis search (i.e. More or less furry couch version
of model)
(d) better semantic matching from crude sketch (ie non-experts!
non-artists)
Research related papers:
(1) How are we doing thing differently than other papers (Zhu)
(2) list of papers: https://github.com/MarkMoHR/Awesome-Sketch-
Based-Applications#4-sketch-based-3d-shape-retrieval

Show current results and visuals.
(1) 2D Sketch retrieval
(2) 3D Sketch SDF retrieval (*ARE WE GOING TO DO THIS OR
JUST 3D MODEL*)
(3) 2D image retrieval
(4) 3D Model retrieval
(5) Text based retrieval
(6) Interpolation of any mode of input including mix. It interpo-
lates codes not inputs.
(7) Sum or Avg of embeddings of any kind and combination of
input based retrieval

Ablations on current results
(1) Smooth Mesh Original Mesh
(2) Blur render versus smoothing mesh Do textures in the render
matter

Show what is achievable with current model
(1) Retrieval by closeness or distance of input.
    (a) Find things along an axis defined by diff of sketch and
target.
        (i) Example: Input sketch and target of text “tall”. Diff of
codes gives a direction vector. You will might need to
have text combine "tall" with the object type you are
manipulating. I.E. "A Tall Chair" + sketch of a chair.
        (ii) multi "text axis" ie "tall chair" vs "short chair" to create
an axis along which to blend towards a particular feature
        (iii) combine multiple inputs using the multi-mode input
methods that are on the todo list. Chair image/sketch
combined with "tall" into a new code. Then subtract the
embedding of the image/sketch to get the axis/dir.
            (A) Extrapolate input code towards target and you should
get taller versions of the input
            (B) Extrapolate away (negative diff) and hopefully you
get shorter things.
(2) Artist control of retrieval by manually weighting multiple
inputs interactively. (BEN)

How to go about using multiple sources of input?
(1) Task description: Retrieval but also Multi-Modal Retrieval:
(2) Input Spec Are we fixing modalities and counts? Or are
we allowing any mix? (ben will look into whether we fix
modalities /counts or not over the weekend)
(3) Datasets:
(a) Shapenet.
(b) Synty
(c) Can we release a subset
(4) Output spec:
(a) How many models do we show?
(5) Metrics.
(a) Text2Mesh uses an R-Similarity Score.
(b) What other metrics are there? (BEN

What data processing do we need?

Dataset
Shapenet Categories:
'04379243': 'table
'04256520': 'sofa'
'03001627': 'chair'
'02958343': 'car'
'02691156': 'plane

Processing:
1. Use the existing pipeline that makes the meshes manifold but loses all materials
2. Just load and render images
3. Just load and render image then post process the images (smooth out features) You will need the render, object mask/depth buffer, albedo.  These will help with the post-processing.


\end{lstlisting}
    
    % \begin{enumerate}
    % \item Show current results and visuals.
    % \item 2D Sketch retrieval
    % \item 3D Sketch SDF retrieval
    % \item 2D image retrieval
    % \item 3D Model retrieval
    % \item Text based retrieval
    % \item Interpolation of any mode of input including mix. It \item interpolates codes not inputs.
    % \item Sum or Avg of embeddings of any kind and combination of input based retrieval
    % \item Show what is achievable with current model
    % \item Retrieval by closeness or distance of input.
    % \item Find things along an axis defined by diff of sketch and target.
    % \item Example: Input sketch and target of text “tall”. Diff of codes gives a direction vector.
    % \item Extrapolate input code towards target and you should get taller versions of the input
    % \item Extrapolate away (negative diff) and hopefully you get shorter things.
    % \item Artist control of retrieval by manually weighting multiple inputs interactively.
    % \item How to go about using multiple sources of input?
    % \item Task description: Retrieval but also Multi-Modal \item \item Retrtieval:
    % Input Spec
    % Are we fixing modalities and counts? Or are we allowing any mix? (ben will look into whether we fix modalities / counts or not over the weekend)
    % \item Datasets:
    % \item Shapenet.
    % \item Synti??? Spelling?
    % \item Can we release a subset
    % \item Output spec:
    % \item How many models do we show?
    % \item Metrics.  
    % \item Text2Mesh uses an R-Similarity Score.
    % \end{enumerate}

story:
we solve a fundamental problem (taking sparse 2d text / image / sketch input and retrieving complex 3d output) impacting downstream tasks (world building)


The ability to use crude 2d sketches and natural language empowers unskilled artists inside a virtual world to author content.  

inside virtual environment modeling is difficult, people want to create things with their hands and voices, 

Here is the story outline of what we are trying to do in the paper and why we think it is important.

\textbf{why is this a problem downstream?} 

3D Content generation has a high barrier to entry given the specialized skills necessary to model by hand. Even with existing 3D modeling software / VR modeling tools - this is both labor intensive and requires highly specialized skill-sets. Foundationally, we observe a disconnect between human understanding and existing (this is obviously an understatement) geometric retrieval based methods... all of which is to say that existing data-driven approaches lack artistic controls, to which end we utilize multi-modality fusion to 'fuse' images (natural and synthetic), sketches, text for our prompts.

\textbf{Valerio:} I would also add some motivation for the multi-modal nature of our approach.

\textbf{what is the actual problem?}

geometric retrievals are fundamentally limited and may require complex machinery for the techniques to work, to say nothing of scalability. CLIP provides a bridge to this gap that we then leverage, by utilizing a pre-trained backbone we are able to extract features which allows us to manipulate the latent space s.t. we get so-called desirable / interesting traits at a higher level of abstraction than traditional geometric algorithms would allow.
This could go in the direction of gradient driven optimizations ala style transfer-like algorithms, but it may also be enough to explore the 2d vs 3d multiple-modal input space as a starting point.

\textbf{what do we do to address this?}

Our approach allows for multi-modal conditional feature driven retrieval through a 3D asset database, consisting of a combination of text, 2D images or sketches and 3D meshes by leveraging pre-trained model weights optimized over 400 million natural images. This embedding space allows "semantic understanding" feature extraction of the images and text passed to it.

\textbf{What's the distilled down novel contribution?}

Other work shows work on stylization of meshes, where we retrieve meshes by a simple sketch (and all these other cool things).

\vspace{2cm}
